Coo: Rethink Data Anomalies In Databases

Transaction processing technology has three important contents: data anomalies, isolation levels, and concurrent control algorithms. Concurrent control algorithms are used to eliminate some or all data anomalies at different isolation levels to ensure data consistency. Isolation levels in the current ANSI standard are defined by disallowing certain kinds of data anomalies. Yet, the definitions of data anomalies in the ANSI standard are controversial. On one hand, the definitions lack a mathematical formalization and cause ambiguous interpretations. On the other hand, the definitions are made in a case-by-case manner and lead to a situation that even a senior DBA could not have infallible knowledge of data anomalies, due to a lack of a full understanding of its nature. While revised definitions in existing literature propose various mathematical formalizations to correct the former argument, how to address the latter argument still remains an open problem. In this paper, we present a general framework called Coo with the capability to systematically define data anomalies. Under this framework, we show that existing reported data anomalies are only a small portion. While we theoretically prove that Coo is complete to mathematically formalize data anomalies, we employ a novel method to classify infinite data anomalies. In addition, we use this framework to define new isolation levels and quantitatively describe the concurrency and rollback rate of mainstream concurrency control algorithms. These works show that the C and I of ACID can be quantitatively analyzed based on all data anomalies.

==> sections/cc_algorithms.tex <==
\section{Data anomaly and CC algorithms}

==> sections/concurrencyModel.tex <==

\begin{table}[ht]
\caption{Analysis of concurrency model with equal probabilities of different conflicts. } \label{tab:concurrency_model}
% \resizebox{\textwidth}{70mm}{
\small
\input{tables/concurrency_model}
% }

\end{table}

\subsection{Concurrency Evaluation Model}\label{sec_ConcurrencyModel}
In this part, we utilize the model defined in section 2 to quantitatively study the characteristic of concurrency control algorithms. As discussed above, the POPs taking the transaction status into account include nine categories, i.e., \{$W_i C_i R_j$\}, \{$W_i C_i W_j$\}, \{$R_i C_i W_j$\}, \{$W_i W_j$, $W_i W_j C_j$\}, \{$W_i R_j$, $W_i R_j C_i$,    $W_i R_j C_j$\}, \{$R_i W_j$, $R_i W_j C_i$, $R_i W_j C_j$, $R_i W_j A_i$\}, \{$W_i R_j A_i$\}, \{$W_i W_j C_i$\}, \{$W_i W_j C_i$\}.Since the last three types of POPs will form a cycle in conflict graph by themselves, we only consider the remained six types of POPs. Suppose the probability of the occurrence of each type of edge is equal, the concurrency is determined by conflict type. 
For the sake of simplicity, we give unit two to weight of each edge. Table \ref{isolation_level_performance} gives the concurrency degree of each concurrency control algorithms based on the conflict edges.  
The CC algorithms gain 2 for the edge if it can handle the POP without locking or aborting. On the contratary, the CC algorithms gain 0 for the the locking or aborting. 
For some situations, the CC algorithms gain 1 as one of the operations are allowed. % Not sure here! Double Check!
For example, the concurrency degree of 2PL is 1/2 as the 2PL permits concurrent on the conflict pairs RR, WCR, WCW, where RR occupies 2/12 and WCR, WCW occupies 4/12 respectively. So, we sum those probabilities of conflict edges and get the concurrency degree of the 2PL as 1/2. 

Our model can be dynamically adjusted to workloads in real world by monitoring the occurrence of POPs by modified the weight of each edge. 
For example, As our experiments show in Table \ref{table:anomaly_statistics} that the anomalies with WW conflicts in syntactic histories occur more than 60$\%$.  We further compute that the POPs of WW in the conflict cycles are the most and more than 30$\%$ among 9 POPs, and it is more than 40$\%$ when only compare to the 6 POPs in the model. So giving the probability of 2/5 instead of 2/12 to WW conflict is more realistic. We adapt these workload dynamics in the model by giving weights and leave this to our future work.


==> sections/isolation_level.tex <==
\section{Data anomaly and isolation level}



==> tables/concurrency_model.tex <==
\begin{tabular}{llllllll}
\toprule
\hline
CC algorithm             & RR & WR      & WW & RW & WCR & WCW & total    \\\hline
2PL          & 2  & 0       &  0  & 0   & 2   & 2   & 6/12  \\\hline
2PL+MVCC     & 2  & 2  & 0  & 1  & 2   & 2   & 8/12  \\\hline
TO           & 2  & 1       & 1  & 1  & 2   & 2   & 9/12  \\\hline
TO+MVCC      & 2  & 2       & 1  & 2  & 2   & 2   & 11/12 \\\hline
OCC+ MVCC    & 2  & 2       & 0   & 2  & 2   & 2   & 10/12 \\\hline

OCC+TO+MVCC  & 2  & 2       & 1  & 2  & 2   & 2   & 11/12 \\\hline
SILO+TO+OCC  & 2  & 1       & 0   & 0   & 2   & 2   & 7/12  \\\hline
SSI+MVCC     & 2  & 2       & 0  & 2  & 2   & 2   & 10/12 \\\hline
% OCC+SSI+MVCC & 2  & 2       & 0   & 2  & 2   & 2   & 10/12 \\\hline
OCC+WSI+MVCC & 2  & 2        & 2 & 0   & 2   & 2   & 10/12  \\\hline
\bottomrule
\end{tabular}
